Hash Function Learning via Codewords

In this paper we introduce a novel hash learning framework that has two main distinguishing features, when compared to past approaches. First, it utilizes codewords in the Hamming space as ancillary means to accomplish its hash learning task. These codewords, which are inferred from the data, attempt to capture similarity aspects of the data's hash codes. Secondly and more importantly, the same framework is capable of addressing supervised, unsupervised and, even, semi-supervised hash learning tasks in a natural manner. A series of comparative experiments focused on content-based image retrieval highlights its performance advantages.

==> TitleAuthors.tex <==
\title{Hash Function Learning via Codewords}

\author{Yinjie Huang\inst{1} \and Michael Georgiopoulos\inst{1} \and \\ Georgios C. Anagnostopoulos\inst{2}}
\institute{University of Central Florida, Department of Electrical Engineering \& Computer Science, 4000 Central Florida Blvd, Orlando, Florida, 32816, USA \\ 
\email{yhuang@eecs.ucf.edu, michaelg@ucf.edu}
\and Florida Institute of Technology, Department of Electrical and Computer Engineering,\\ 150 W University Blvd, Melbourne, Florida,  32901, USA \\
\email{georgio@fit.edu}}

\maketitle

% You may provide any keywords that you 
% find helpful for describing your paper; these are used to populate 
% the "keywords" metadata in the PDF but will not be shown in the document

\vskip 0.3in
